MJ-Bench: Is Your Multimodal Reward Model Really a Good Judge for Text-to-Image Generation?

While text-to-image models like DALLE-3 and Stable Diffusion are rapidly proliferating, they often encounter challenges such as hallucination, bias, and the production of unsafe, low-quality output. To effectively address these issues, it is crucial to align these models with desired behaviors based on feedback from a multimodal judge. Despite their significance, current multimodal judges frequently undergo inadequate evaluation of their capabilities and limitations, potentially leading to misalignment and unsafe fine-tuning outcomes. To address this issue, we introduce MJ-Bench, a novel benchmark which incorporates a comprehensive preference dataset to evaluate multimodal judges in providing feedback for image generation models across four key perspectives: alignment, safety, image quality, and bias. Specifically, we evaluate a large variety of multimodal judges including smaller-sized CLIP-based scoring models, open-source VLMs (e.g. LLaVA family), and close-source VLMs (e.g. GPT-4o, Claude 3) on each decomposed subcategory of our preference dataset. Experiments reveal that close-source VLMs generally provide better feedback, with GPT-4o outperforming other judges in average. Compared with open-source VLMs, smaller-sized scoring models can provide better feedback regarding text-image alignment and image quality, while VLMs provide more accurate feedback regarding safety and generation bias due to their stronger reasoning capabilities. Further studies in feedback scale reveal that VLM judges can generally provide more accurate and stable feedback in natural language (Likert-scale) than numerical scales. Notably, human evaluations on end-to-end fine-tuned models using separate feedback from these multimodal judges provide similar conclusions, further confirming the effectiveness of MJ-Bench. All data, code, models are available at https://huggingface.co/MJ-Bench.

==> content/checklist.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{See abstract and the introduction section}
  \item Did you describe the limitations of your work?
    \answerYes{See the discussion section.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{The paper conforms to all guidelines.}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{No theoretical contents or results.}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{No theoretical contents or results.}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Code and data are released with the submission.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Details are specified.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNo{No substantial amount of compute is consumed for this work.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{All existing assets are properly cited.}
  \item Did you mention the license of the assets?
    \answerYes{All licenses are properly mentioned if needed.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{New assets are released via URL and explained in the supplemental material.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNo{The data was generated by AI models.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{The nature of the potential offensive content is discussed.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerYes{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerYes{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNo{}
\end{enumerate}

\end{enumerate}

==> content/data_sheet.tex <==
\section{Data sheet}
\label{app:datasheet}
We follow the documentation frameworks provided by \citet{datasheet}.

\subsection{Motivation}

\paragraph{For what purpose was the dataset created?}

\begin{itemize}[leftmargin=1.3em,topsep=1pt,noitemsep]
    \item Our dataset aims to provide a holistic evaluation of the existing multimodal reward models as judge to provide feedback for text-to-image models.
    \item Our dataset is consisted of four major subsets that include the evaluations for text-image alignment, safety, image quality (aesthetics), and bias.
\end{itemize}

\paragraph{Who created the dataset (e.g., which team, research group) and on behalf of which entity (e.g., company, institution, organization)?}
\begin{itemize}[leftmargin=1.3em,topsep=1pt,noitemsep]
\item Our dataset is jointly developed by a collaborative effort from the following research groups:
\begin{itemize}
\item University of North Carolina at Chapel Hill
\item University of Chicago
\item Stanford University
\item University of California, Santa Cruz
\item Duke University
\item ESSEC Business School
\item Illinois Institute of Technology
\item University of California, San Diego
\item University of Queensland
\item Stony Brook University
\end{itemize}
\end{itemize}


\subsection{Composition/collection process/preprocessing/cleaning/labeling and uses:}

\begin{itemize}[leftmargin=1.3em,topsep=1pt,noitemsep]
\item We detail the data collection and processing process in this paper.
\end{itemize}

\subsection{Distribution}

\paragraph{Will the dataset be distributed to third parties outside of the entity (e.g., company, institution, organization) on behalf of which the dataset was created?}

\begin{itemize}[leftmargin=1.3em,topsep=1pt,noitemsep]
\item No. Our dataset will be managed and maintained by our research group.
\end{itemize}

\paragraph{How will the dataset be distributed (e.g., tarball on website, API, GitHub)?}

\begin{itemize}[leftmargin=1.3em,topsep=1pt,noitemsep]
\item The dataset and leaderboard will be released to the public and hosted on Huggingface at \url{https://huggingface.co/spaces/MJ-Bench} and the evaluation toolkit will be hosted on GitHub at \url{https://github.com/BillChan226/MJ-Bench}.
\end{itemize}.

\paragraph{When will the dataset be distributed?}

\begin{itemize}[leftmargin=1.3em,topsep=1pt,noitemsep]
\item We have already released the dataset.
\end{itemize}

\paragraph{Will the dataset be distributed under a copyright or other intellectual property (IP) license, and/or under applicable terms of use (ToU)?}

\begin{itemize}[leftmargin=1.3em,topsep=1pt,noitemsep]
\item Our dataset will be distributed under the CC BY 4.0 license.
\end{itemize}


\subsection{Maintenance}

\paragraph{How can the owner/curator/manager of the dataset be contacted (e.g., email address)?}

\begin{itemize}[leftmargin=1.3em,topsep=1pt,noitemsep]
\item Please contact Zhaorun Chen (\texttt{zhaorun@uchicago.edu}) and Prof. Huaxiu Yao (\texttt{huaxiu@cs.unc.edu}), who are responsible for maintenance.
\end{itemize}



\paragraph{Will the dataset be updated (e.g., to correct labeling errors, add new instances, delete instances)?}


\begin{itemize}[leftmargin=1.3em,topsep=1pt,noitemsep]
\item Yes, if additional tasks are included or any errors are discovered, we will correct the dataset and update the results on the leaderboard accordingly. These updates will be reflected on our website.
\end{itemize}

\paragraph{If others want to extend/augment/build on/contribute to the dataset, is there a mechanism for them to do so?}

For dataset contributions and evaluation modifications, the most efficient method is through GitHub pull requests. Additionally, you can contact the corresponding authors via email for assistance.



==> material/obsolete_bias.tex <==

\begin{table}[t]
    \centering
    \caption{Result for Bias.}
    \resizebox{1.0\linewidth}{!}{%
    \begin{tabular}{c|cccccccccccc|cccccccc}
    \toprule
         & \multicolumn{12}{c}{\bf Occupation} & \multicolumn{8}{c}{\bf Education} \\
         & \multicolumn{2}{c}{Age} & \multicolumn{2}{c}{Gender} & \multicolumn{2}{c}{Race} & \multicolumn{2}{c}{Nationality} & \multicolumn{2}{c}{Religion} & \multicolumn{2}{c}{\cellcolor{skyblue}Avg} & \multicolumn{2}{c}{Gender} & \multicolumn{2}{c}{Race} & \multicolumn{2}{c}{Nationality} & \multicolumn{2}{c}{\cellcolor{skyblue}Avg} \\
         & NDS & GES & NDS & GES & NDS & GES & NDS & GES & NDS & GES & NDS & GES & NDS & GES & NDS & GES & NDS & GES & NDS & GES \\
         \midrule
         CLIP-v1$^\diamondsuit$ & - & - & - & - & - & - & - & - & - & - & \cellcolor{skyblue} - & \cellcolor{skyblue} - & - & - & - & - & - & - & \cellcolor{skyblue} - & \cellcolor{skyblue} - \\
         BLIP-v2$^\diamondsuit$ & - & - & - & - & - & - & - & - & - & - & \cellcolor{skyblue} - & \cellcolor{skyblue} - & - & - & - & - & - & - & \cellcolor{skyblue} - & \cellcolor{skyblue} - \\
         PickScore-v1$^\diamondsuit$ & - & - & - & - & - & - & - & - & - & - & \cellcolor{skyblue} - & \cellcolor{skyblue} - & - & - & - & - & - & - & \cellcolor{skyblue} - & \cellcolor{skyblue} - \\
         HPS-v2.1$^\diamondsuit$ & - & - & - & - & - & - & - & - & - & - & \cellcolor{skyblue} - & \cellcolor{skyblue} - & - & - & - & - & - & - & \cellcolor{skyblue} - & \cellcolor{skyblue} - \\
         ImageReward$^\diamondsuit$ & - & - & - & - & - & - & - & - & - & - & \cellcolor{skyblue} - & \cellcolor{skyblue} - & - & - & - & - & - & - & \cellcolor{skyblue} - & \cellcolor{skyblue} - \\
         Aesthetics$^\diamondsuit$ & - & - & - & - & - & - & - & - & - & - & \cellcolor{skyblue} - & \cellcolor{skyblue} - & - & - & - & - & - & - & \cellcolor{skyblue} - & \cellcolor{skyblue} - \\
         \midrule
         LLaVA-1.5-7b$^\heartsuit$ & - & - & - & - & - & - & - & - & - & - & \cellcolor{skyblue} - & \cellcolor{skyblue} - & - & - & - & - & - & - & \cellcolor{skyblue} - & \cellcolor{skyblue} - \\
         LLaVA-1.5-13b$^\heartsuit$ & - & - & - & - & - & - & - & - & - & - & \cellcolor{skyblue} - & \cellcolor{skyblue} - & - & - & - & - & - & - & \cellcolor{skyblue} - & \cellcolor{skyblue} - \\
         LLaVA-1.6-mistral-7b$^\heartsuit$ & - & - & - & - & - & - & - & - & - & - & \cellcolor{skyblue} - & \cellcolor{skyblue} - & - & - & - & - & - & - & \cellcolor{skyblue} - & \cellcolor{skyblue} - \\
         LLaVA-1.6-vicuna-7b$^\heartsuit$ & - & - & - & - & - & - & - & - & - & - & \cellcolor{skyblue} - & \cellcolor{skyblue} - & - & - & - & - & - & - & \cellcolor{skyblue} - & \cellcolor{skyblue} - \\
         LLaVA-1.6-34b$^\heartsuit$ & - & - & - & - & - & - & - & - & - & - & \cellcolor{skyblue} - & \cellcolor{skyblue} - & - & - & - & - & - & - & \cellcolor{skyblue} - & \cellcolor{skyblue} - \\
         Internvl-chat-v1-2$^\heartsuit$ & - & - & - & - & - & - & - & - & - & - & \cellcolor{skyblue} - & \cellcolor{skyblue} - & - & - & - & - & - & - & \cellcolor{skyblue} - & \cellcolor{skyblue} - \\
         Internvl-chat-v1-5$^\heartsuit$ & - & - & - & - & - & - & - & - & - & - & \cellcolor{skyblue} - & \cellcolor{skyblue} - & - & - & - & - & - & - & \cellcolor{skyblue} - & \cellcolor{skyblue} - \\
         Instructblip-7b$^\heartsuit$ & - & - & - & - & - & - & - & - & - & - & \cellcolor{skyblue} - & \cellcolor{skyblue} - & - & - & - & - & - & - & \cellcolor{skyblue} - & \cellcolor{skyblue} - \\
         MiniGPT4-v2$^\heartsuit$ & - & - & - & - & - & - & - & - & - & - & \cellcolor{skyblue} - & \cellcolor{skyblue} - & - & - & - & - & - & - & \cellcolor{skyblue} - & \cellcolor{skyblue} - \\
         Qwen-VL-Chat$^\spadesuit$ & - & - & - & - & - & - & - & - & - & - & \cellcolor{skyblue} - & \cellcolor{skyblue} - & - & - & - & - & - & - & \cellcolor{skyblue} - & \cellcolor{skyblue} - \\
         Qwen-VL-Max$^\spadesuit$ & - & - & - & - & - & - & - & - & - & - & \cellcolor{skyblue} - & \cellcolor{skyblue} - & - & - & - & - & - & - & \cellcolor{skyblue} - & \cellcolor{skyblue} - \\
         Idefics2-8b$^\spadesuit$ & - & - & - & - & - & - & - & - & - & - & \cellcolor{skyblue} - & \cellcolor{skyblue} - & - & - & - & - & - & - & \cellcolor{skyblue} - & \cellcolor{skyblue} - \\
         Prometheus-Vision-13b$^\spadesuit$ & - & - & - & - & - & - & - & - & - & - & \cellcolor{skyblue} - & \cellcolor{skyblue} - & - & - & - & - & - & - & \cellcolor{skyblue} - & \cellcolor{skyblue} - \\
         \midrule
         GPT-4-vision$^\clubsuit$ & - & - & - & - & - & - & - & - & - & - & \cellcolor{skyblue} - & \cellcolor{skyblue} - & - & - & - & - & - & - & \cellcolor{skyblue} - & \cellcolor{skyblue} - \\
         Gemini Ultra$^\clubsuit$ & - & - & - & - & - & - & - & - & - & - & \cellcolor{skyblue} - & \cellcolor{skyblue} - & - & - & - & - & - & - & \cellcolor{skyblue} - & \cellcolor{skyblue} - \\
         Claude 3 Opus$^\clubsuit$ & - & - & - & - & - & - & - & - & - & - & \cellcolor{skyblue} - & \cellcolor{skyblue} - & - & - & - & - & - & - & \cellcolor{skyblue} - & \cellcolor{skyblue} - \\
    \bottomrule
    \end{tabular}%
    }
    \label{exp:main_result}
\end{table}


==> material/obsolete_main.tex <==

\begin{table}[t]
    \centering
    \caption{Main result.}
    \resizebox{1.0\linewidth}{!}{%
    \begin{tabular}{c|ccc|ccc|ccc|ccc|c}
    \toprule
         & \multicolumn{3}{c}{\bf Alignment} & \multicolumn{3}{c}{\bf Safety} & \multicolumn{3}{c}{\bf Artifact} & \multicolumn{3}{c}{\bf Bias} & {\bf Overall} \\
         & Easy & Hard & \cellcolor{skyblue}Avg & NSFW & Toxicity & \cellcolor{skyblue}Avg & Distortion & Blurry & \cellcolor{skyblue}Avg & Occupation & Education & \cellcolor{skyblue}Avg & Avg \\
         \midrule
         CLIP-v1$^\diamondsuit$ & - & -  & \cellcolor{skyblue} - & - & - & \cellcolor{skyblue} - & - & - & \cellcolor{skyblue} - & - & - & \cellcolor{skyblue} - &  - \\
          BLIP-v2$^\diamondsuit$ & - & - & \cellcolor{skyblue} - & - & - & \cellcolor{skyblue} - & - & - & \cellcolor{skyblue} - & - & - & \cellcolor{skyblue} - &  - \\
          PickScore-v1$^\diamondsuit$ & - & - & \cellcolor{skyblue} - & - & - & \cellcolor{skyblue} - & - & - & \cellcolor{skyblue} - & - & - & \cellcolor{skyblue} - &  - \\
          HPS-v2.1$^\diamondsuit$ & - & - & \cellcolor{skyblue} - & - & - & \cellcolor{skyblue} - & - & - & \cellcolor{skyblue} - & - & - & \cellcolor{skyblue} - &  - \\
          ImageReward$^\diamondsuit$ & - & - & \cellcolor{skyblue} - & - & - & \cellcolor{skyblue} - & - & - & \cellcolor{skyblue} - & - & - & \cellcolor{skyblue} - &  - \\
          Aesthetics$^\diamondsuit$ & - & - & \cellcolor{skyblue} - & - & - & \cellcolor{skyblue} - & - & -  & \cellcolor{skyblue} - & - & -  & \cellcolor{skyblue} - &  - \\
          \midrule
          LLaVA-1.5-7b$^\heartsuit$ & - & - & \cellcolor{skyblue} - & - & - & \cellcolor{skyblue} - & - & - & \cellcolor{skyblue} - & - & - & \cellcolor{skyblue} - &  - \\
          LLaVA-1.5-13b$^\heartsuit$ & - & - & \cellcolor{skyblue} - & - & - & \cellcolor{skyblue} - & - & - & \cellcolor{skyblue} - & - & -  & \cellcolor{skyblue} - &  - \\
          LLaVA-1.6-mistral-7b$^\heartsuit$ & - & - & \cellcolor{skyblue} - & - & - & \cellcolor{skyblue} - & - &  - & \cellcolor{skyblue} - & - & - & \cellcolor{skyblue} - &  - \\
          LLaVA-1.6-vicuna-7b$^\heartsuit$ & - & - & \cellcolor{skyblue} - & - & - & \cellcolor{skyblue} - & - & - & \cellcolor{skyblue} - & - & - & \cellcolor{skyblue} - &  - \\
          LLaVA-1.6-34b$^\heartsuit$ & - & - & \cellcolor{skyblue} - & - & - & \cellcolor{skyblue} - & - & - & \cellcolor{skyblue} - & - & -  & \cellcolor{skyblue} - &  - \\
          Instructblip-7b$^\heartsuit$ & - & - & \cellcolor{skyblue} - & - & - & \cellcolor{skyblue} - & - & - & \cellcolor{skyblue} - & - & - & \cellcolor{skyblue} - &  - \\
          MiniGPT4-v2$^\heartsuit$ & - & - & \cellcolor{skyblue} - & - & - & \cellcolor{skyblue} - & - & - & \cellcolor{skyblue} - & - & - & \cellcolor{skyblue} - &  - \\
          Qwen-VL-Chat$^\spadesuit$ & - & - & \cellcolor{skyblue} - & - & - & \cellcolor{skyblue} - & - & - & \cellcolor{skyblue} - & - & - & \cellcolor{skyblue} - &  - \\
          Internvl-chat-v1-5$^\spadesuit$ & - & - & \cellcolor{skyblue} - & - & - & \cellcolor{skyblue} - & - & - & \cellcolor{skyblue} - & - & - & \cellcolor{skyblue} - &  - \\
          Idefics2-8b$^\spadesuit$ & - & - & \cellcolor{skyblue} - & - & - & \cellcolor{skyblue} - & - & - & \cellcolor{skyblue} - & - & - & \cellcolor{skyblue} - &  - \\
        Prometheus-Vision-13b$^\spadesuit$ & - & - & \cellcolor{skyblue} - & - & - & \cellcolor{skyblue} - & - & - & \cellcolor{skyblue} - & - & - & \cellcolor{skyblue} - &  - \\
          \midrule
          GPT-4-vision$^\clubsuit$ & - & - & \cellcolor{skyblue} - & - & - & \cellcolor{skyblue} - & - & - & \cellcolor{skyblue} - & - & - & \cellcolor{skyblue} - &  - \\
          GPT-4o$^\clubsuit$ & - & - & \cellcolor{skyblue} - & - & - & \cellcolor{skyblue} - & - & - & \cellcolor{skyblue} - & - & - & \cellcolor{skyblue} - &  - \\
          Gemini Ultra$^\clubsuit$ & - & - & \cellcolor{skyblue} - & - & - & \cellcolor{skyblue} - & - & - & \cellcolor{skyblue} - & - & - & \cellcolor{skyblue} - &  - \\
          Claude 3 Opus$^\clubsuit$ & - & - & \cellcolor{skyblue} - & - & - & \cellcolor{skyblue} - & - & - & \cellcolor{skyblue} - & - & - & \cellcolor{skyblue} - &  - \\
    \bottomrule
    \end{tabular}%
    }
    \label{exp:main_result}
\end{table}


==> table/original_scale_study.tex <==
\begin{table}[t]
    \centering
    \caption{Result with different scale.}
    \resizebox{1.0\linewidth}{!}{%
    \begin{tabular}{c|cc|cc|cc|cc}
    \toprule
         & \multicolumn{2}{c}{\bf Alignment} & \multicolumn{2}{c}{\bf Safety} & \multicolumn{2}{c}{\bf Artifact} & \multicolumn{2}{c}{\bf Bias} \\
         & numeric & likert  & numeric & likert  & numeric & likert & numeric & likert\\
          \midrule
          LLaVA-1.5-7b$^\heartsuit$ & - & - & - & - & - & - & - & - \\
          LLaVA-1.5-13b$^\heartsuit$ & - & - & - & - & - & - & - & -  \\
          LLaVA-NeXT-mistral-7b$^\heartsuit$ & - & - & - & - & - & - & - & -  \\
          LLaVA-NeXT-vicuna-7b$^\heartsuit$ & - & - & - & - & - & - & - & -\\
          Instructblip-7b$^\heartsuit$ & - & - & - & - & - & - & 57.4 & 85.8  \\
          MiniGPT4-v2$^\heartsuit$ & - & - & - & - & - & - & - & -\\
          Prometheus-Vision-13b$^\heartsuit$ & - & - & - & - & - & - & - & -  \\
          Qwen-VL-Chat$^\spadesuit$ & - & - & - & - & - & - & - & - \\
          Internvl-chat-v1-5$^\spadesuit$ & - & - & - & - & - & - & 65.3 & 83.5  \\
          Idefics2-8b$^\spadesuit$ & - & - & - & - & - & - & 52.7 & 77.6 \\
          \midrule
          GPT-4-vision$^\clubsuit$ & - & - & - & - & - & - & 80.4 & 93.2  \\
          GPT-4o$^\clubsuit$ & - & - & - & - & - & - & 82.5 & 92.8 \\
          Gemini Ultra$^\clubsuit$ & - & - & - & - & - & - & 75.3 & 88.6 \\
          Claude 3 Opus$^\clubsuit$ & - & - & - & - & - & - & 65.6 & 85.0  \\
    \bottomrule
    \end{tabular}%
    }
    \label{exp:numeric_likert}
\end{table}


==> table/temp_table.tex <==
\begin{table}[t]
    \centering
    \caption{Main result.}
    \resizebox{1.0\linewidth}{!}{%
    \begin{tabular}{c|cc|cc|cc|ccc}
    \toprule
         & \multicolumn{2}{c}{\bf Alignment} & \multicolumn{2}{c}{\bf Safety} & \multicolumn{2}{c}{\bf Artifact} & \multicolumn{3}{c}{\bf Bias} \\
         & Avg w. tie & Avg w.o. Tie & Avg w. tie & Avg w.o. Tie & Avg w. tie & Avg w.o. Tie & ACC & NDS & GES \\
    \midrule
         CLIP-v1$^\diamondsuit$ & $44.0$ & $60.7$ & $13.1$ & $25.7$ & $41.9$ & $82.7$ & 57.4 & 76.3 & 86.9 \\
         BLIP-v2$^\diamondsuit$ & $21.5$ & $34.1$ & $44.3$ & $75.3$ & $7.8$ & $24.4$ & 68.7 & 83.7 & 91.3 \\
         PickScore-v1$^\diamondsuit$ & $60.9$ & $65.9$ & $37.3$ & $41.3$ & $83.9$ & $92.2$ & 31.0 & 66.5 & 81.1 \\
         HPS-v2.1$^\diamondsuit$ & $48.8$ & $73.6$ & $20.8$ & $35.7$ & $69.6$ & $99.1$ & 55.0 & 77.9 & 87.6 \\
         ImageReward$^\diamondsuit$ & $51.1$ & $67.9$ & $24.9$ & $35.9$ & $63.5$ & $91.7$ & 40.9 & 73.7 & 85.3 \\
         Aesthetics$^\diamondsuit$ & $34.8$ & $56.7$ & $31.6$ & $54.7$ & $70.8$ & $98.5$ & 61.4 & 85.7 & 92.1 \\
    \midrule
         LLaVA-1.5-7b$^\heartsuit$ & $22.0$ & $50.8$ & - & - & - & - & 83.7 & 70.4 & 88.7 \\
         LLaVA-1.5-13b$^\heartsuit$ & $10.3$ & $51.9$ & - & - & - & - & 69.7 & 74.3 & 88.6 \\
         LLaVA-NeXT-mistral-7b$^\heartsuit$ & - & - & - & - & - & - & 69.9 & 64.3 & 85.4 \\
         LLaVA-NeXT-vicuna-13b$^\heartsuit$ & - & - & - & - & - & - & 56.3 & 64.0 & 82.7 \\
         Instructblip-7b$^\heartsuit$ & - & - & - & - & - & - & 53.1 & 80.8 & 91.2 \\
         MiniGPT4-v2$^\heartsuit$ & - & - & - & - & - & - & 32.6 & 67.0 & 83.3 \\
         Prometheus-Vision-7b$^\heartsuit$ & - & - & - & - & - & - & 49.5 & 43.4 & 74.4 \\
         Prometheus-Vision-13b$^\heartsuit$ & - & - & - & - & - & - & 66.3 & 46.3 & 76.8 \\
         Qwen-VL-Chat$^\heartsuit$ & $31.1$ & $31.6$ & - & - & - & - & 71.9 & 62.8 & 86.2 \\
         Internvl-chat-v1-5$^\heartsuit$ & $75.8$ & $77.6$ & - & - & - & - & 25.4 & 69.6 & 84.3 \\
         Idefics2-8b$^\heartsuit$ & $32.6$ & $43.5$ & - & - & - & - & 42.1 & 58.7 & 79.4 \\
     \midrule
         Qwen-VL-Chat$^\spadesuit$ & $31.1$ & $31.6$ & - & - & - & - & 71.9 & 62.8 & 86.2 \\
         Internvl-chat-v1-5$^\spadesuit$ & $75.8$ & $77.6$ & - & - & - & - & 25.4 & 69.6 & 84.3 \\
         Idefics2-8b$^\spadesuit$ & $32.6$ & $43.5$ & - & - & - & - & 42.1 & 58.7 & 79.4 \\
         GPT-4-vision$^\clubsuit$ & - & - & - & - & - & - & 79.0 & 80.4 & 93.2 \\
         GPT-4o$^\clubsuit$ & - & - & - & - & - & - & 65.8 & 82.5 & 92.8 \\
         Gemini Ultra$^\clubsuit$ & - & - & - & - & - & - & 55.6 & 75.3 & 88.6 \\
         Claude 3 Opus$^\clubsuit$ & - & - & - & - & - & - & 57.7 & 65.6 & 85.0 \\
    \bottomrule
    \end{tabular}%
    }
    % \label{exp:main_result}
\end{table}
